KnowMe Paper Radar: Lightweight Discovery of Promising Papers in the Age of Autoresearch

Large language models (LLMs) are pushing research toward semi-automation: ideas turn into preprints ever faster, and autoresearch pipelines add papers of uneven rigor. When a technique can be overtaken within months, citations arrive too late to tell which new papers deserve reading, so strong work goes unnoticed and newcomers lose their bearings. Yet from the day it appears, a preprint carries the track records of the people and institutions behind it. Established researchers guard their reputations and choose problems and collaborators with research taste, so their involvement tends to raise a paper's quality floor. Building on this signal, we present KnowMe Paper Radar, a lightweight arXiv discovery tool that weights each paper's topical relevance by the reputation its authors and institutions stake on it. Author credit also diffuses by message passing along collaborations to surface rising stars, and institutions are profiled through the researchers they hold in each direction rather than by headcount. In a sealed test on 10,386 new papers, those with an identity-bound author were twice as likely to reach the top tenth of early citations. As its library grows into a scholarly knowledge graph that research agents can query through a command-line interface (CLI), KnowMe also offers a promising literature entry point for future autoresearch and recursive self-improvement (RSI).

==> analysis/revision_v59/links/FIGURE_ARXIV_LINKS.tex <==
% Native, invisible, exact-filename link overlays for the current native figures.
% Load once after graphicx/hyperref, near the end of the preamble.
% Original graphics and all their box dimensions remain unchanged.
\RequirePackage{graphicx}
\RequirePackage{xparse}
\makeatletter
\newsavebox{\KM@graphicbox}
\newdimen\KM@gw \newdimen\KM@gh
\newdimen\KM@lx \newdimen\KM@ly \newdimen\KM@lw \newdimen\KM@lh
\newcommand{\KM@arxivhotspot}[5]{%
  \KM@lx=#1\KM@gw\relax
  \KM@ly=#2\KM@gh\relax
  \advance\KM@ly by -\dp\KM@graphicbox
  \KM@lw=#3\KM@gw\relax
  \KM@lh=#4\KM@gh\relax
  \rlap{\kern\KM@lx\raisebox{\KM@ly}[0pt][0pt]{\hbox{%
    \pdfannot width \KM@lw height \KM@lh depth 0pt {%
      /Subtype /Link /Border [0 0 0] /H /I
      /A << /S /URI /URI (https://arxiv.org/abs/#5) >>
    }%
  }}}%
}

\expandafter\def\csname KM@arxiv@analysis/method_trace_primary_v41/figures/atlas_trace_primary_v41.pdf\endcsname{%
  \KM@arxivhotspot{0.6619658120}{0.7834271240}{0.0945313413}{0.0241666540}{2609.23697}%
  \KM@arxivhotspot{0.6619658120}{0.7528715685}{0.0945313413}{0.0241666540}{2609.14193}%
  \KM@arxivhotspot{0.6619658120}{0.5889826796}{0.0945313413}{0.0241666751}{2605.30880}%
  \KM@arxivhotspot{0.6619658120}{0.5584271240}{0.0945313413}{0.0241666751}{2605.01489}%
  \KM@arxivhotspot{0.6619658120}{0.3945382351}{0.0945313413}{0.0241666751}{2608.25593}%
  \KM@arxivhotspot{0.6619658120}{0.3639826796}{0.0945313413}{0.0241666751}{2607.15557}%
  \KM@arxivhotspot{0.2425036406}{0.0848160129}{0.1132594997}{0.0241666328}{2510.21903v2}%
}

\expandafter\def\csname KM@arxiv@analysis/visual_assets_v37/figures/landscape_compact_v37.pdf\endcsname{%
  \KM@arxivhotspot{0.1539696848}{0.7698908185}{0.1105508690}{0.0375230214}{2605.20025v2}%
  \KM@arxivhotspot{0.7593382746}{0.7698908185}{0.1092821561}{0.0375230214}{2606.11926v1}%
  \KM@arxivhotspot{0.1539696848}{0.5913193899}{0.1105508690}{0.0375230214}{2601.14525v1}%
  \KM@arxivhotspot{0.7586705395}{0.5913193899}{0.1105508527}{0.0375230214}{2606.09833v2}%
}

\expandafter\def\csname KM@arxiv@analysis/revision_v61/figures/figure20_genmem_current_v61.pdf\endcsname{%
  \KM@arxivhotspot{0.0720641063}{0.8695919770}{0.1151132421}{0.0326923004}{2609.34633v1}%
}

\expandafter\def\csname KM@arxiv@analysis/revision_v61/figures/figure21_rrsi_current_v61.pdf\endcsname{%
  \KM@arxivhotspot{0.0720641063}{0.8695919770}{0.1151132421}{0.0326923004}{2609.24972v3}%
}

\expandafter\def\csname KM@arxiv@analysis/revision_v61/figures/figure22_kimi_current_v61.pdf\endcsname{%
  \KM@arxivhotspot{0.0720641063}{0.8695919770}{0.1151132421}{0.0326923004}{2607.24653v2}%
}

\let\KM@originalincludegraphics\includegraphics
\RenewDocumentCommand{\includegraphics}{s O{} m}{%
  \ifcsname KM@arxiv@\detokenize{#3}\endcsname
    \begingroup
      \sbox{\KM@graphicbox}{%
        \IfBooleanTF{#1}{\KM@originalincludegraphics*[#2]{#3}}{\KM@originalincludegraphics[#2]{#3}}%
      }%
      \KM@gw=\wd\KM@graphicbox
      \KM@gh=\dimexpr\ht\KM@graphicbox+\dp\KM@graphicbox\relax
      \leavevmode\hbox{%
        \csname KM@arxiv@\detokenize{#3}\endcsname
        \usebox{\KM@graphicbox}%
      }%
    \endgroup
  \else
    \IfBooleanTF{#1}{\KM@originalincludegraphics*[#2]{#3}}{\KM@originalincludegraphics[#2]{#3}}%
  \fi
}
\makeatother

